Topological complexity of n points on a tree

The topological complexity of a path-connected space $X,$ denoted $TC(X),$ can be thought of as the minimum number of continuous rules needed to describe how to move from one point in $X$ to another. The space $X$ is often interpreted as a configuration space in some real-life context. Here, we consider the case where $X$ is the space of configurations of $n$ points on a tree $\Gamma.$ We will be interested in two such configuration spaces. In the, first, denoted $C^n(\Gamma),$ the points are distinguishable, while in the second, $UC^n(\Gamma),$ the points are indistinguishable. We determine $TC(UC^n(\Gamma))$ for any tree $\Gamma$ and many values of $n,$ and consequently determine $TC(C^n(\Gamma))$ for the same values of $n$ (provided the configuration spaces are path-connected).

==> 160802-Scheirer arXiv/Labeling/LabeledFigures.tex <==

\def\VertexOrdering{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $\ast$ at 181 36
\pinlabel $1$ at 189 95
\pinlabel $2$ at 181 162
\pinlabel $3$ at 150 153
\pinlabel $4$ at 117 173
\pinlabel $5$ at 91 188
\pinlabel $6$ at 223 161
\pinlabel $7$ at 274 190
\pinlabel $8$ at 241 231
\pinlabel $9$ at 223 261
\pinlabel $10$ at 206 290
\pinlabel $11$ at 309 249
\pinlabel $12$ at 332 288
\pinlabel $13$ at 286 348
\pinlabel $14$ at 270 386
\pinlabel $15$ at 330 400
\pinlabel $16$ at 345 321
\pinlabel $17$ at 359 354
\pinlabel $18$ at 369 384
\endlabellist
\centering
\includegraphics[height=4.5cm]{Labeling/VertexOrderingNoLabels}
\caption{The ordering of the vertices on a tree $\Gamma$}
\label{fig:VertexOrdering}
\end{figure}
}

\def\AllowableOrientations{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $v$ at 211 227
\pinlabel $v$ at 593 227
\pinlabel $\ast$ at 175 15
\pinlabel $\ast$ at 557 15
\endlabellist
\centering
\includegraphics[height=4.5cm]{Labeling/AllowableOrientationsNoLabels}
\caption{Two collections of arcs in a graph $\Gamma$}
\label{fig:AllowableOrientations}
\end{figure}
}

\def\Cells{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $e$ at 192 133
\pinlabel $3$ at 132 130
\pinlabel $10$ at 550 272
\pinlabel $9$ at 566 243
\pinlabel $f$ at 940 300
\pinlabel $16$ at 1000 300
\endlabellist
\centering
\includegraphics[height=4.5cm]{Labeling/CellsNoLabels}
\caption{Three different cells in $UD^2(\Gamma)$}
\label{fig:Cells}
\end{figure}
}

\def\CriticalCells{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $\ast$ at 125 20
\endlabellist
\centering
\includegraphics[height=4.5cm]{Labeling/CriticalCellNoLabels}
\caption{A critical 3-cell $c$ in $UD^8(\Gamma)$}
\label{fig:CriticalCells}
\end{figure}
}

\def\Clouds{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $1$ at 168 82
\pinlabel $1$ at 105 170
\pinlabel $0$ at 233 160
\pinlabel $2$ at 221 244
\pinlabel $0$ at 291 240
\pinlabel $1$ at 262 330
\pinlabel $0$ at 308 348
\pinlabel $0$ at 333 333
%%%%%
\pinlabel $1$ at 498 82
\pinlabel $1$ at 435 170
\pinlabel $0$ at 563 160
\pinlabel $2$ at 551 244
\pinlabel $2$ at 621 240
%%%%%
\pinlabel $0$ at 828 82
\pinlabel $1$ at 767 170
\pinlabel $0$ at 897 160
\pinlabel $2$ at 885 244
\pinlabel $3$ at 955 240
\endlabellist
\centering
\includegraphics[height=4.5cm]{Labeling/CloudExampleNoLabels}
\caption{Cloud diagrams for classes $[c],$ with $c$ as in Figure \ref{fig:CriticalCells} (left), $[d]$ (middle), and $[d']$ (right)}
\label{fig:Clouds}
\end{figure}
}

\def\PartOneA{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $\ast$ at 140 36
\pinlabel$A_1$ at 170 84 
\pinlabel $A_2$ at 196 201
\pinlabel $A_3$ at 305 240
\pinlabel $v_1$ at 139 127
\pinlabel $v_2$ at 173 147
\pinlabel $v_3$ at 154 209
\pinlabel $v_4$ at 257 175
\pinlabel $v_5$ at 244 253
\pinlabel $v_6$ at 206 287
\pinlabel $v_7$ at 308 280
\pinlabel $v_8$ at 283 159
\pinlabel $v_9$ at 315 129
\pinlabel $v_{10}$ at 356 133
\pinlabel $v_{11}$ at 338 70
%%%%%
\pinlabel $u_1$ at 494 131
\pinlabel $e_1$ at 524 104
\pinlabel $u_2$ at 536 154
\pinlabel $e_2$ at 576 134
\pinlabel $u_3$ at 508 176
\pinlabel $e_3$ at 546 199
\pinlabel $u_4$ at 598 186
\pinlabel $e_4$ at 625 171
\pinlabel $u_5$ at 581 243
\pinlabel $e_5$ at 637 237
\pinlabel $u_6$ at 536 265
\pinlabel $e_6$ at 572 290
\pinlabel $u_7$ at 671 290
\pinlabel $e_7$ at 668 256
\pinlabel $u_8$ at 653 133
\pinlabel $e_8$ at 628 142
\pinlabel $u_9$ at 684 162
\pinlabel $e_9$ at 684 128
\pinlabel $u_{10}$ at 715 161
\pinlabel $e_{10}$ at 724 126
\pinlabel $u_{11}$ at 706 69
\pinlabel $e_{11}$ at 668 78
\pinlabel $\ast=w_1$ at 503 33
\pinlabel $w_2$ at 564 228
\pinlabel $w_3$ at 694 242
\pinlabel $w_4$ at 522 60
\pinlabel $w_5$ at 522 75
%%%%%
\pinlabel $u'_1$ at 860 131
\pinlabel $e'_1$ at 890 104
\pinlabel $u'_2$ at 934 161
\pinlabel $e'_2$ at 917 120
\pinlabel $u'_3$ at 874 176
\pinlabel $e'_3$ at 912 199
\pinlabel $u'_4$ at 964 187
\pinlabel $e'_4$ at 990 174
\pinlabel $u'_5$ at 947 239
\pinlabel $e'_5$ at 1003 237
\pinlabel $u'_6$ at 904 260
\pinlabel $e'_6$ at 938 290
\pinlabel $u'_7$ at 1037 290
\pinlabel $e'_7$ at 1034 250
\pinlabel $u'_8$ at 1019 131
\pinlabel $e'_8$ at 992 142
\pinlabel $u'_9$ at 1050 156
\pinlabel $e'_9$ at 1050 124
\pinlabel $u'_{10}$ at 1081 165
\pinlabel $e'_{10}$ at 1090 126
\pinlabel $u'_{11}$ at 1072 96
\pinlabel $e'_{11}$ at 1030 80
\pinlabel $w'_1$ at 1010 48
\pinlabel $w'_2$ at 878 265
\pinlabel $w'_3$ at 1124 160
\pinlabel $\ast=w'_4$ at 869 33
\pinlabel $w'_5$ at 888 60
\endlabellist
\centering
\includegraphics[height=4cm]{Labeling/part1aNoLabels}
\caption{A graph $\Gamma$ (left) and the critical cells $\Phi$ and $\Psi$ in $UD^{27}(\Gamma)$ (center and right)}
\label{fig:PartOneA}
\end{figure}
}

\def\PartOneB{
\begin{figure}[h]
\labellist
\scriptsize\hair 2pt
\pinlabel $10$ at 252 234
\pinlabel $8$ at 325 307
\pinlabel $8$ at 367 163
%%%%%
\pinlabel $8$ at 815 234
\pinlabel $8$ at 892 307
\pinlabel $10$ at 936 163
\endlabellist
\centering
\includegraphics[height=4cm]{Labeling/part1bNoLabels}
\caption{Cloud representations for $[c_4]$ (left) and $[d_4]$ (right) corresponding to the cells $\Phi$ and $\Psi$ in $UD^{27}(\Gamma)$}
\label{fig:PartOneB}
\end{figure}
}

\def\PartTwoA{
\begin{figure}[h!]
\labellist
\tiny\hair 2pt
\pinlabel $u_1$ at 190 217
\pinlabel $e_1$ at 260 191
\pinlabel $u_2$ at 416 228
\pinlabel $e_2$ at 422 181
\pinlabel $\widetilde{u}_1$ at 109 141
\pinlabel $\widetilde{e}_1$ at 180 142
\pinlabel $\widetilde{u}_2$ at 155 300
\pinlabel $\widetilde{e}_2$ at 212 295
\pinlabel $\widetilde{u}_3$ at 285 268
\pinlabel $\widetilde{e}_3$ at 315 216
%%%%%
\pinlabel $u'_1$ at 804 232
\pinlabel $e'_1$ at 787 162
\pinlabel $u'_2$ at 984 222
\pinlabel $e'_2$ at 944 172
\pinlabel $\widetilde{u}_4$ at 829 352
\pinlabel $\widetilde{e}_4$ at 906 336
\pinlabel $\widetilde{u}_5$ at 770 384
\pinlabel $\widetilde{e}_5$ at 809 431
\pinlabel $\widetilde{u}_6$ at 921 426
\pinlabel $\widetilde{e}_6$ at 958 376
\endlabellist
\centering
\includegraphics[height=3.7cm]{Labeling/part2aNoLabels}
\caption{The critical cells $\Phi$ and $\Psi$ in $UD^{10}(\Gamma)$}
\label{fig:PartTwoA}
\end{figure}
}

\def\PartTwoBi{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $A_1$ at 154 86
\pinlabel $A_2$ at 176 177
\pinlabel $A_3$ at 276 227
\pinlabel $V_1$ at 109 90
\pinlabel $V_2$ at 137 201
\pinlabel $V_3$ at 288 271
\pinlabel $V_1'$ at 316 55
\pinlabel $V_2'$ at 191 275
\pinlabel $V_3'$ at 365 135
\pinlabel $\widetilde{V}_1$ at 249 169
\pinlabel $\widetilde{V}_2$ at 228 239
\pinlabel $\widetilde{V}_3$ at 269 159
\pinlabel $\widehat{V}_1$ at 155 137
\pinlabel $\widehat{V}_2$ at 302 116
%%%%%
\pinlabel $U_1$ at 478 115
\pinlabel $E_1$ at 510 93
\pinlabel $U_2$ at 494 168
\pinlabel $E_2$ at 530 188
\pinlabel $U_3$ at 652 280
\pinlabel $E_3$ at 650 240
\pinlabel $\widetilde{U}_1$ at 579 177
\pinlabel $\widetilde{E}_1$ at 611 163
\pinlabel $\widetilde{U}_2$ at 564 230
\pinlabel $\widetilde{E}_2$ at 616 217
\pinlabel $\widetilde{U}_3$ at 639 118
\pinlabel $\widetilde{E}_3$ at 608 130
\pinlabel $\widehat{U}_1$ at 518 147
\pinlabel $\widehat{E}_1$ at 551 151
\pinlabel $\widehat{U}_2$ at 667 152
\pinlabel $\widehat{E}_2$ at 670 115
%%%%%
\pinlabel $U'_1$ at 1054 82
\pinlabel $E'_1$ at 1034 51
\pinlabel $U'_2$ at 888 250
\pinlabel $E'_2$ at 916 280
\pinlabel $U'_3$ at 1093 145
\pinlabel $E'_3$ at 1063 118
\pinlabel $\widetilde{U}_1$ at 942 177
\pinlabel $\widetilde{E}_1$ at 974 163
\pinlabel $\widetilde{U}_2$ at 930 230
\pinlabel $\widetilde{E}_2$ at 976 217
\pinlabel $\widetilde{U}_3$ at 1002 146
\pinlabel $\widetilde{E}_3$ at 968 130
\pinlabel $\widehat{U}_1'$ at 914 154
\pinlabel $\widehat{E}_1'$ at 898 108
\pinlabel $\widehat{U}_2'$ at 1028 145
\pinlabel $\widehat{E}_2'$ at 1005 106
\endlabellist
\centering
\includegraphics[height=4cm]{Labeling/part2biNoLabels}
\caption{The critical cells $\Phi$ and $\Psi$ in $UD^{16}(\Gamma)$ (middle and right)}
\label{fig:PartTwoBi}
\end{figure}
}

\def\PartTwoBii{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $A_1$ at 154 82
\pinlabel $A_2$ at 176 177
\pinlabel $A_0$ at 291 227
\pinlabel $V_1$ at 111 89
\pinlabel $V_2$ at 142 190
\pinlabel $V'_1$ at 313 50
\pinlabel $V'_2$ at 190 268
\pinlabel $\widetilde{V}_1$ at 252 168
\pinlabel $\widetilde{V}_2$ at 233 232
\pinlabel $\widetilde{V}_3$ at 288 266
\pinlabel $\widetilde{V}_4$ at 273 152
\pinlabel $\widetilde{V}_5$ at 361 129
\pinlabel $\widehat{V}_1$ at 163 130
\pinlabel $\widehat{V}_2$ at 302 111
%%%%%
\pinlabel $U_1$ at 479 112
\pinlabel $E_1$ at 507 87
\pinlabel $U_2$ at 499 162
\pinlabel $E_2$ at 532 187
\pinlabel $\widetilde{U}_1$ at 580 170
\pinlabel $\widetilde{E}_1$ at 612 158
\pinlabel $\widetilde{U}_2$ at 583 240
\pinlabel $\widetilde{E}_2$ at 616 214
\pinlabel $\widetilde{U}_3$ at 652 274
\pinlabel $\widetilde{E}_3$ at 652 236
\pinlabel $\widetilde{U}_4$ at 638 114
\pinlabel $\widetilde{E}_4$ at 611 130
\pinlabel $\widetilde{U}_5$ at 700 147
\pinlabel $\widetilde{E}_5$ at 727 121
\pinlabel $\widehat{U}_1$ at 519 138
\pinlabel $\widehat{E}_1$ at 561 118
\pinlabel $\widehat{U}_2$ at 666 144
\pinlabel $\widehat{E}_2$ at 673 112
\pinlabel $x$ at 680 250
%%%%%
\pinlabel $U'_1$ at 1054 80
\pinlabel $E'_1$ at 1037 52
\pinlabel $U'_2$ at 882 244
\pinlabel $E'_2$ at 916 275
\pinlabel $\widetilde{U}_1$ at 942 170
\pinlabel $\widetilde{E}_1$ at 974 158
\pinlabel $\widetilde{U}_2$ at 945 240
\pinlabel $\widetilde{E}_2$ at 976 212
\pinlabel $\widetilde{U}_3$ at 1014 274
\pinlabel $\widetilde{E}_3$ at 1014 236
\pinlabel $\widetilde{U}_4$ at 1000 145
\pinlabel $\widetilde{E}_4$ at 972 130
\pinlabel $\widetilde{U}_5$ at 1064 149
\pinlabel $\widetilde{E}_5$ at 1089 121
\pinlabel $\widehat{U}'_1$ at 918 147
\pinlabel $\widehat{E}'_1$ at 899 104
\pinlabel $\widehat{U}'_2$ at 1030 139
\pinlabel $\widehat{E}'_2$ at 1004 105
\pinlabel $x'$ at 1095 153
\endlabellist
\centering
\includegraphics[height=4cm]{Labeling/part2biiNoLabels}
\caption{The critical cells $\Phi$ and $\Psi$ in $UD^{19}(\Gamma)$ (middle and right)}
\label{fig:PartTwoBii}
\end{figure}
}

\def\RCv{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $e$ at 182 321
\pinlabel $0$ at 124 284
\pinlabel $1$ at 158 382
\pinlabel $C_\tau$ at 220 400
\pinlabel $3$ at 280 352
\pinlabel $1$ at 258 294
\pinlabel $C_\iota$ at 209 248
\pinlabel $0$ at 410 274
\pinlabel $2$ at 313 153
%%%%%
\pinlabel $0$ at 557 284
\pinlabel $2$ at 600 382
\pinlabel $C_\tau\cup\{\tau(e)\}$ at 653 410
\pinlabel $3$ at 717 352
\pinlabel $1$ at 691 294
\pinlabel $C_\iota\cup\{\iota(e)\}$ at 642 248
\pinlabel $0$ at 843 278
\pinlabel $2$ at 746 153
\endlabellist
\centering
\includegraphics[height=5cm]{Labeling/RCvNoLabels}
\caption{The cloud diagram $\mathcal{C}$ for a standard cocycle $\phi_{[c]}$ (left) and the cloud diagram for the cochain $\mathcal{R}_{\mathcal{C},v}$ (right)}
\label{fig:RCv}
\end{figure}
}

\def\ThetaTau{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $0$ at 104 280
\pinlabel $1$ at 148 332
\pinlabel $3$ at 194 300
\pinlabel $1$ at 196 256
\pinlabel $0$ at 340 266
\pinlabel $2$ at 244 140
%%%%%
\pinlabel $0$ at 439 280
\pinlabel $2$ at 483 324
\pinlabel $2$ at 540 306
\pinlabel $1$ at 531 256
\pinlabel $0$ at 675 266
\pinlabel $2$ at 579 140
\endlabellist
\centering
\includegraphics[height=4cm]{Labeling/ThetaTauNoLabels}
\caption{The sum $\sum_{i=1}^{d(v)-1}\Theta_{\mathcal{C},v,\tau,i}$ with $\mathcal{C}$ as in Figure \ref{fig:RCv}}
\label{fig:ThetaTau}
\end{figure}
}

\def\ThetaIota{
\begin{figure}[h]
\labellist
\tiny\hair 2pt
\pinlabel $0$ at 100 284
\pinlabel $2$ at 148 332
\pinlabel $3$ at 194 300
\pinlabel $0$ at 196 256
\pinlabel $0$ at 340 266
\pinlabel $2$ at 244 140
%%%%%
\pinlabel $0$ at 449 280
\pinlabel $2$ at 493 324
\pinlabel $3$ at 550 306
\pinlabel $0$ at 541 256
\pinlabel $0$ at 685 266
\pinlabel $2$ at 589 140
%%%%%
\pinlabel $0$ at 802 280
\pinlabel $2$ at 843 324
\pinlabel $3$ at 900 306
\pinlabel $0$ at 896 256
\pinlabel $0$ at 1035 266
\pinlabel $2$ at 941 140
\endlabellist
\centering
\includegraphics[height=4cm]{Labeling/ThetaIotaNoLabels}
\caption{The sum $\sum_{i=1}^{d(v)-1}\Theta_{\mathcal{C},v,\iota,i}$ with $\mathcal{C}$ as in Figure \ref{fig:RCv}}
\label{fig:ThetaIota}
\end{figure}
}
